Leveraging Recursive Gumbel-Max Trick for Approximate Inference in Combinatorial Spaces

Structured latent variables allow incorporating meaningful prior knowledge into deep learning models. However, learning with such variables remains challenging because of their discrete nature. Nowadays, the standard learning approach is to define a latent variable as a perturbed algorithm output and to use a differentiable surrogate for training. In general, the surrogate puts additional constraints on the model and inevitably leads to biased gradients. To alleviate these shortcomings, we extend the Gumbel-Max trick to define distributions over structured domains. We avoid the differentiable surrogates by leveraging the score function estimators for optimization. In particular, we highlight a family of recursive algorithms with a common feature we call stochastic invariant. The feature allows us to construct reliable gradient estimates and control variates without additional constraints on the model. In our experiments, we consider various structured latent variable models and achieve results competitive with relaxation-based counterparts.

==> tables/overview.tex <==
\begin{table*}[h!]
\centering
\caption{Similarly to the perturbed input $\exprv$, the trace $\tracerv$ has tractable score function, yet the score function estimator yields lower variance. Such estimator is a practical alternative to an estimator using $\structrv$, since the score of $\structrv$ involves computationally demanding marginalization. Additionally, $\exprv$ admits conditional reparameterization given $\tracerv$.}
\label{table:overview}
\begin{tabular}{lccc}
\toprule
& Input $\exprv$
& Execution Trace $\tracerv = \tracerv(\exprv)$
& Output $\structrv = \structrv(\tracerv)$
\\
\midrule
Score $\nabla_{\expparam} \log \mathbb P(\cdot)$
& Tractable
& Tractable
& Intractable
\\
REINFORCE variance
& High
& Moderate
& Low
%\\
%Entropy $H(\cdot)$
%& Tractable
%& Sample Estimates
%& Intractable
\\
Conditional $p_\exprv(\exprv \mid \cdot)$
& $\delta(\exprv - \expreal)$
& $\sum \operatorname{Exp} (\sum \expparam_k)$
& Intractable
\\
\bottomrule
\end{tabular}
\end{table*}


==> tables/tablesTopKOriginal.tex <==

\newcommand{\corrtopk}[1]{\hlmyred{#1}}
\newcommand{\topk}[1]{\hlmyblue{#1}}
\newcommand{\both}[1]{\hlmypurple{#1}}

\begin{table*}[t]
  \centering
  \label{fig:l2x:review}
  \caption{For $k$-subset selection on aroma aspect,  tend to outperform baseline relaxations. Test set MSE ($\times 10^{-2}$) and subset precision (\%) is shown for models selected on valid. MSE. Bottom:  (red) selects contiguous words while \emph{Top $k$} (blue) picks scattered words.}  
  \begin{small}
  \begin{tabular}{@{}llcccccc@{}}
  \toprule
   & & \multicolumn{2}{c}{$k=5$} &  \multicolumn{2}{c}{$k=10$} &  \multicolumn{2}{c}{$k=15$} \\
   \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
  Model & Relaxation & MSE & Subs. Prec. &  MSE & Subs. Prec. &  MSE & Subs. Prec. \\
  \midrule
  \multirow{7}{*}{\shortstack[l]{Simple}}
  & \emph{L2X} \citep{chen2018learning}
  	& $3.6 \pm  0.1$ 
  	& $28.3 \pm 1.7$  
  	& $3.0 \pm  0.1$ 
  	& $25.5 \pm 1.2$ 
  	& $2.6 \pm  0.1$ 
  	& $25.5 \pm 0.4$ \\
  & \emph{SoftSub} \citep{xie2019reparameterizable}
  	& $3.6 \pm  0.1$ 
  	& $27.2 \pm 0.7$ 
  	& $3.0 \pm  0.1$ 
  	& $26.1 \pm 1.1$ 
  	& $2.6 \pm  0.1$ 
  	& $25.1 \pm 1.0$ \\
  \cmidrule[0.15pt]{2-8}
  & \emph{Euclid. Top $k$}
  	& $3.5 \pm 0.1$ 
  	& $25.8 \pm 0.8$ 
  	& $2.8 \pm  0.1$ 
  	& $32.9 \pm 1.2$ 
  	& $2.5 \pm  0.1$ 
  	& $29.0 \pm 0.3$ \\
  & \emph{Cat. Ent. Top $k$}
  	& $3.5 \pm 0.1$ 
  	& $26.4 \pm 2.0$ 
  	& $2.9 \pm  0.1$ 
  	& $32.1 \pm 0.4$ 
  	& $2.6 \pm  0.1$ 
  	& $28.7 \pm 0.5$ \\
  & \emph{Bin. Ent. Top $k$}
  	& $3.5 \pm  0.1$ 
  	& $29.2 \pm 2.0$ 
  	& $2.7 \pm  0.1$ 
  	& $33.6 \pm 0.6$ 
  	& $2.6 \pm  0.1$ 
  	& $28.8 \pm 0.4$ \\
  & \emph{E.F. Ent. Top $k$}
  	& $3.5 \pm  0.1$ 
  	& $28.8 \pm 1.7$ 
  	& $2.7 \pm  0.1$ 
  	& $32.8 \pm 0.5$ 
  	& $2.5 \pm  0.1$ 
  	& $29.2 \pm 0.8$ \\
  \cmidrule[0.15pt]{2-8}
  & \emph{Corr. Top $k$} 
  	& $\mathbf{2.9 \pm 0.1}$ 
  	& $\mathbf{63.1  \pm 5.3}$ 
  	& $\mathbf{2.5 \pm 0.1}$ 
  	& $\mathbf{53.1 \pm 0.9}$ 
  	& $\mathbf{2.4 \pm 0.1}$ 
  	& $\mathbf{45.5 \pm 2.7}$ \\
  \cmidrule[0.15pt]{1-8}
  \multirow{7}{*}{\shortstack[l]{Complex}}
  & \emph{L2X} \citep{chen2018learning}
  	& $2.7 \pm 0.1$ 
  	& $50.5 \pm 1.0$ 
  	& $2.6 \pm 0.1$ 
  	& $44.1 \pm 1.7$ 
  	& $2.4 \pm 0.1$ 
  	& $44.4 \pm 0.9$ \\
  & \emph{SoftSub} \citep{xie2019reparameterizable}
  	& $2.7 \pm 0.1$ 
  	& $57.1 \pm 3.6$ 
  	& $\mathbf{2.3 \pm 0.1}$ 
  	& $50.2 \pm 3.3$ 
  	& $2.3 \pm 0.1$ 
  	& $43.0 \pm 1.1$ \\
  \cmidrule[0.15pt]{2-8}
  & \emph{Euclid. Top $k$}
  	& $2.7 \pm 0.1$ 
  	& $61.3 \pm 1.2$ 
  	& $2.4 \pm 0.1$ 
  	& $52.8 \pm 1.1$ 
  	& $2.3 \pm 0.1$ 
  	& $44.1 \pm 1.2$ \\
  & \emph{Cat. Ent. Top $k$}
  	& $2.7 \pm 0.1$ 
  	& $61.9 \pm 1.2$ 
  	& $\mathbf{2.3 \pm 0.1}$ 
  	& $52.8 \pm 1.0$ 
  	& $2.3 \pm 0.1$ 
  	& $44.5 \pm 1.0$ \\
  & \emph{Bin. Ent. Top $k$}
  	& $2.6 \pm 0.1$ 
  	& $62.1 \pm 0.7$ 
  	& $\mathbf{2.3 \pm 0.1}$ 
  	& $50.7 \pm 0.9$ 
  	& $2.3 \pm 0.1$ 
  	& $44.8 \pm 0.8$ \\
  & \emph{E.F. Ent. Top $k$}  	
  	& $2.6 \pm 0.1$ 
  	& $59.5 \pm 0.9$ 
  	& $\mathbf{2.3 \pm 0.1}$ 
  	& $54.6 \pm 0.6$ 
  	& $2.2 \pm 0.1$ 
  	& $44.9 \pm 0.9$ \\
  \cmidrule[0.15pt]{2-8}
  & \emph{Corr. Top $k$} 
  	& $\mathbf{2.5 \pm 0.1}$ 
  	& $\mathbf{67.9 \pm 0.6}$ 
  	& $\mathbf{2.3 \pm 0.1}$ 
  	& $\mathbf{60.2 \pm 1.3}$ 
  	& $\mathbf{2.1 \pm 0.1}$ 
  	& $\mathbf{57.7 \pm 3.8}$ \\
  \bottomrule
  \end{tabular}
  \end{small}
\end{table*}
